Effective Estimation of Contact Force and Torque for Vision-based Tactile Sensor with Helmholtz-Hodge Decomposition

Retrieving rich contact information from robotic tactile sensing has been a challenging, yet significant task for the effective perception of object properties that the robot interacts with. This work is dedicated to developing an algorithm to estimate contact force and torque for vision-based tactile sensors. We first introduce the observation of the contact deformation patterns of hyperelastic materials under ideal single-axial loads in simulation. Then based on the observation, we propose a method of estimating surface forces and torque from the contact deformation vector field with the Helmholtz-Hodge Decomposition (HHD) algorithm. Extensive experiments of calibration and baseline comparison are followed to verify the effectiveness of the proposed method in terms of prediction error and variance. The proposed algorithm is further integrated into a contact force visualization module as well as a closed-loop adaptive grasp force control framework and is shown to be useful in both visualization of contact stability and minimum force grasping task.

==> sections/acknowledgment.tex <==
\section*{Acknowledgment}


==> sensor_design_and_fabrication.tex <==
% !TeX spellcheck = en_GB
\section{FingerVision Design and Fabrication}


This section introduces the conceptual design of FingerVision, followed by fabrication process in detail.

\subsection{Conceptual Design}


The basic scheme to get contact information from optical-based tactile sensor is by inducing large
deformation of material in contact region for camera to capture the deformation. Similar to \cite{yamaguchi2016combining}, our sensor consists of elastomer with embedded markers, camera and supporting frame.  Although the tactile sensor developed in \cite{yamaguchi2016combining} is versatile on sensing multiple modalities, the relatively low stability during real robotic action makes
their sensor not an ideal tactile component for robots. In the work of \cite{dong2017improved}, Gelsight sensor is compact,
easy to use, able to reconstruct super fine contact surface, however, extra calibration of correspondence between color and surface normal is required. 
Our sensor design emphasizes on stability, durability, readiness to use and adopts optical-based sensor scheme for its superior properties. 

\begin{figure}
	\centering
	\includegraphics[width=0.46\textwidth]{diagram_render_and_finish.png}
	\caption{Design and fabrication of FingerVision tactile sensor. (a). Conceptual diagram of sensor. (b). Finish of tactile sensor. (c). Fabrication process. (c). Rendered model of sensor supporting frame. (d). Casting in action with frame in mold. (e). Intermediate step after markers attached.}
\end{figure}


For the design of optical-based tactile sensor, the following issues need to be taken into account. 
\begin{itemize}
	\item \textit{Functionality}. To enhance the stability of markers tracking, consistent background and even illumination are critical. Wide view angle fisheye is necessary because large view field is needed given short focusing range.
	\item \textit{Number
of components}. Large number of components increases degree of difficulty during fabrication process and augments the complexity of system, which requires more characteristics to be set properly.
	\item \textit{Compactness}. Compactness of sensor determines whether it can be installed on robot fingers and limits the range of tasks it can be applied to.
\end{itemize}
 
Conceptual design of FingerVision is depicted in Fig. 1(a). Fisheye camera, a transparent elastic
layer, and the supporting frame comprise the hardware of the sensor. Inside the elastomer,
markers are used as tracking feature points reflecting the displacement of material in
neighborhood, and with a compact 2D marker array, dense displacement field of contact
surface can be acquired. We choose fisheye as transducer due to the relative larger field of view,
which achieves a better trade-off between the compactness of sensor and large sensing area. 
High tracking stability is guaranteed with even illumination, rather than the way of light guiding through acrylic plate as reported in \cite{yuan2015measurement}, in our design, the LED light source
is put outside of white supporting frame (via 3D printing), and the light transmits through the resin
with large diffusion , which consequently illuminates the sensing area evener. Unlike the design in \cite{yamaguchi2016combining}, we coat the gel layer with another reflective layer to block external light sources that can deteriorate the tracking
performance of sensor. Similarly, the supporting frame is designed to be fully enclosed to increase tracking stability. 

Fig. 1(c) and (d) show the rendered 3D model of sensor frame and mold for the casting
of Gel layer respectively. After iterations of design, fabrication and redesign, it is found that
distributed locking holes in the outer ridge of frame are also important to maintain firm attachment between silicone rubber layer and the frame, learned from \cite{yamaguchi2017implementing}.


\subsection{Fabrication}



Our fabrication process includes three steps as shown below, in addition, material and components are also described.

1) \textit{3D printing of sensor frame and casting mold}. Benefiting from the easily available 3D printing, we are able to accelerate the prototyping process. The sensor frame and
mold are made of Epoxy Resin with SLA 3D printing technology,
possessing properties of smooth surface finish, good accuracy, and mechanical strength. 

2) \textit{Elastomer casting and marker embedding}. As for material of the elastomer, we
choose a transparent silicone rubber \textit{Solaris} from Smooth-On, Inc. This material, come
with two parts, A and B, and cures with weight ratio of \textit{1A:1B}. The casting lasts for 24 hours in room temperature and can be accelerated in the oven, the shore hardness of cured
silicone rubber is 15A. To put markers on the surface, the markers are patterned on a water transfer paper
first, and follow the product instruction to transfer ink from paper to gel surface. In this manner,
the markers density is much higher than that of the method used in \cite{yamaguchi2016combining} by
embedding plastic beads into the elastic layer. Fig. 1(d) shows the casting of sensor prototype in action.

3) \textit{Assembly of sensor components}. The camera we use is a commercially available CCD web
camera with fisheye lens. Before the camera is installed on the frame,
fisheye camera calibration is required. Here we adopt chessboard camera calibration method for
fisheye lens to estimate intrinsic matrix. Since the working focus range of camera is short compared to other application scenarios, calibration chessboard needs to be printed with small size as well.
After these three steps, we obtain the optical-based tactile sensor as shown in Fig. 1(b).

==> sensor_signal_processing.tex <==
% !TeX spellcheck = en_GB
\section{Sensor Signal Processing}

\begin{figure}
	\centering
	\includegraphics[width=0.48\textwidth]{data_processing_flow.png}
	\caption{Sensor data processing pipeline and corresponding results (with sensor pressed by thumb). (a). Captured input image. (b). Key points detection result. (c). Marker tracking vectors. (d). Interpolated marker displacement field.}
\end{figure}



After acquiring images of contact region, additional processing is conducted to obtain contact deformation field. Fig. 2 shows the signal acquisition and processing pipeline with results step-by-step. Markers detection,
tracking algorithm and deformation field interpolation are three essential components of
the system. For the markers are 2D array of black dots on a lighter background, we adopt
blob detection to calculate centers of every black dots. With fully enclosed chamber and even illumination, the blob detection works stably with fine-tuned parameters. A sample image and its key points are shown in
Fig. 2(a) and (b). Compared with transparent sensing elastomer design in \cite{yamaguchi2016combining}, our sensor outperforms in terms of robustness in various working scene.

\begin{algorithm}
	
	\caption{Markers Tracking Algorithm}
	
	\begin{algorithmic}
		
		\WHILE {TRUE}
		\STATE Capture image
		\STATE $centroids \gets blobDetection(image)$
		\IF {First loop}
		\STATE $T, initPos \gets centroids$ 
		\STATE Continue
		
		\ELSE 
		\STATE $C \gets KNN(initPos, centroids)$
		
		\FOR {$k \gets 1$ \TO  $N$}
		\STATE $lastPoint \gets T_k$
		\STATE $currentPoint \gets C(lastPoint)$
		%			\STATE 
		
		\IF {$dist(lastPoint, currentPoint) \leq d$}
		\STATE Update lastPoint in T with currentPoint
		\ENDIF
		\ENDFOR
		\ENDIF
		
		
		\ENDWHILE
	\end{algorithmic}
\end{algorithm}


Recovering of deformation field requires tracking of markers sequentially on time domain. After the centroids of markers are obtained in marker detection module, we proceed to
track the movement of every marker individually. Commonly there are two approaches for tracking problems, one is by updating correspondences between consecutive frames and then tracing back to the initial frame to obtain displacements, another is by registering correspondences of markers between first frame and current frame. For registration methodology, the state-of-the-art of non-rigid registration methods are
coherent points drift method ( CPD) \cite{myronenko2007non} and elastic Iterative Closet Points (ICP) \cite{stewart2003dual} method. Although registration methods is able to compute correspondences between arbitrary two frames, which makes it more robust and less interdependent between frame to frame, the iterative optimization scheme severely deteriorates the real-time sensing capability.  



Therefore, we adopt the scheme of updating correspondences frame by frame, and the tracking algorithm with
tolerance to markers detection failure is developed. Firstly K-nearest neighborhood
method is used to obtain nearest points correspondences $C$ between previous frame and
current frame, and then corresponded pairs with euclidean distance larger than manually set threshold $d$ are rejected, which is reasonable by assuming that the displacements of points are small
with the short time elapsed between consecutive frames. Thereafter, valid point
correspondences are updated in tracking matrix $T$ as latest correspondence matrix
associating initial marker positions and that of last updated markers. 



Deformation of elastic material is naturally smooth with its low pass filter effect for external excitation. 
Therefore, to further increase the density of deformation field and obtain
vector field with fixed size in fixed locations to facilitate further usages, we perform displacement
field interpolation based on the tracked displacement vectors. Here radius basis function (RBF) interpolation
method is selected to obtain smooth interpolation with relatively lower computation cost. The interpolation result is shown in Fig. 2. The frame rate of our set up (Intel Core i7-7700K@4.2GHz, 8 cores) with the processing algorithm is 15 FPS, which is adequate for various robotic tasks.

\begin{figure}
	\centering
	\includegraphics[width=0.45\textwidth]{response_three_excitation.png}
	\caption{Deformation field and orthogonal projection when excited with different directional forces (Colormap to value: Green: neutral, Red: positive, Blue: negative). (a). Applied with Normal force. (b). Applied with normal and tangential force. (c). Applied with normal and rotational force along contact surface normal.}
\end{figure}


Contact motion can be decomposed into normal pressing, tangential translation,
torsional motion. However, in real life, contact breaking happens when pure tangential force is applied without normal pressing. Fig. 3 shows the deformation field obtained with FingerVision sensor while being excited by pure normal, tangential coupled with normal, and torsional coupled with normal forces with a doom shape indent head. It is obvious that our sensor signal can distinguish different contact forces successfully, which is useful for various robot manipulation tasks. Application to slip detection is implemented in next section and it is shown to be effective.



==> slip_detection.tex <==
% !TeX spellcheck = en_GB
\section{Slip Detection}
In this section, we propose a learning based slip detection framework making use of contact deformation field generated by FingerVision sensor. The framework is demonstrated to accurately classify contact into slip and non-slip states using tactile information only.
\subsection{Model Description}


\begin{figure*}
	\centering
	\includegraphics[width=0.7\textwidth, height=3.5cm]{diagram_NN.png}
	\caption{The architecture of slip detection framework using convolutional LSTM network and FingerVision Data.}
\end{figure*}

The architecture of slip detection framework is shown in Fig. 4. Knowing that slip occurrence is a spatiotemporal event on the contact surface, we adopt convolutional LSTM for its capability of capturing spatiotemporal features transition simultaneously \cite{shi1506convolutional}. Compared to the structure concatenating time distributed CNN with LSTM as \cite{li2018slip}, convolutional LSTM network is preferred because spatial feature extraction parameters (convolution kernel weights) are also the hidden node parameters and back propagation update is performed on both domains simultaneously. Besides, the well-performing CNN used in \cite{li2018slip} Inception V3 model contains over 7 million parameters \cite{canziani2016analysis}, which makes the forward pass computation too demanding for real-time implementation. In this perspective, It is alleviating that our model has drastically lower 269,826 parameters. We feed 10 frames of multi-channel images containing deformation field with x axis projection, y axis projection, and magnitude value jointly into convolutional LSTM network sequentially. Since the multiplication operation in common LSTM is replaced by convolutional operation \cite{shi1506convolutional}, the output of LSTM is also 3D tensors. The output of convolutional LSTM is flatten and fed to fully connected layer (FC layer) afterwards. LSTM layer with 64 hidden nodes with $5\times5$ kernal size is set for our model. Multiple layer LSTM structure is beneficial for long term dependency learning, however, considering our data is collected in a relatively short period, single layer structure is constructed. Finally, the FC layer outputs two variables representing the probability of stable contact or slip. 


As for the training setup, Pytorch package is used to build the network and our model is trained on Nvidia GeForce 1060 (6GB graphic memory). In the training phase, The network weights are initialized with random small values and we choose two classes cross entropy as loss function. Adam optimizer with learning rate of $1\times10^{-5}$ is used for network parameters update.  



\subsection{Experimental Analysis}

\begin{figure}
	\centering
	\includegraphics[width=0.45\textwidth]{dataset_objects.png}
	\caption{12 daily objects used in dataset collection.}
\end{figure}

\textbf{Data collection}. To distinguish between slip happening and stable contact, we take advantage of the intuitive human sense of slip since there are no other more reliable artificial slip sensing solutions available except for success/failure labelling of grasp as been implemented in \cite{li2018slip}, \cite{calandra2017feeling}, which is derivative results of slip or stable contact. For data collection, 12 daily objects are used as shown in Fig. 5. Objects comes in different size, shape and material. During every collection, an object is pressed against sensor surface by human hand, then force are applied to objects to generate target motion in a certain period. The labelling of a specific data is determined by human feeling of slip, translational and rotational slip are included and incipient slip is also labelled into slip category. Every raw data contains 15 frames of $30\times30$ pixel interpolated deformation field images (3-channels: dx, dy and magnitude) with an acquisition rate of 15 HZ. The sensor is fixed on a table during data collection to avoid false labelling. Fig. 6 shows an example of data collection with USB flash disk being the contact object. 




In our work, a relative small size of dataset is first manually collected and further slicing to increase dataset volume is performed. Total amount of 1600 data with 800 slip class and 800 non-slip data are obtained. By slicing out subsets from raw data as in \cite{li2018slip}, we increase the dataset size by 5 times to 8000. Five subsets with each containing 10 successive frames are selected out of raw data using a sliding window with stride of 1 frame. As for dataset splitting, 90\% of data is used for training and 10\% for testing. 

\begin{figure}
	\centering
	\includegraphics[width=0.45\textwidth, height=3cm]{data_collection_sample.png}
	\caption{An example of data collection process with USB flash disk. The first row are images recorded by another external camera monitoring the whole process (notes that images in first row are not accurately synchronized to images in later rows). The last 3 rows are magnitude, x axis projection, y axis projection of deformation field respectively.}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=0.45\textwidth, height=4cm]{training_process.png}
	\caption{The network model training process.}
\end{figure}

\textbf{Results analysis}. From training history plotted in Fig. 7, we can see that our prediction accuracy on testing dataset rises over 95\% in first 1000 steps with batch size of 32, equivalent to a training time of 6m23s under our hardware setting. \cite{li2018slip} and \cite{van2018slip} are recent works similar to our paper, Table 1 presents a comparison between the performance of our method and these works in terms of accuracy. According to the testing results, our model using sequential frames of interpolated contact deformation field shows higher accuracy than other works. Furthermore, with a much lower input resolution and relatively shallower network structure, our forward pass time is as low as 0.014 seconds, making it a suitable framework to satisfy real-time requirements of robotic manipulation tasks with mobile computing devices. On another perspective, the performance also shows the effectiveness of our tactile sensor on tracking of contact events. For robot grasping problem, our sensor with proper algorithms can surely improve robot performance by providing dynamic spatiotemperal awareness of contact events.


\begin{table}
	\centering
	\caption{Slip detection accuracy of different works. Highest accuracy in each experiments are used.}
	\begin{tabular}{|c|c|c|}
		\hline 
		\textbf{Input} & \textbf{Framework} & \textbf{Accuracy} \\ 
		\hline 
		Interpolated deformation field (image) & ConvLSTM & \textbf{97.62\%} \\
		\hline 
		Tactile and external image \cite{li2018slip} & CNN+LSTM & 88.03\% \\
		\hline 
		Spectral univariate signals \cite{van2018slip} & LSTM & 94.5\% \\ 
		\hline 
		 
%		\hline 
	\end{tabular} 
	
	
\end{table}



